PACE: Human and Camera Motion Estimation from in-the-wild Videos

We present a method to estimate human motion in a global scene from moving cameras. This is a highly challenging task due to the coupling of human and camera motions in the video. To address this problem, we propose a joint optimization framework that disentangles human and camera motions using both foreground human motion priors and background scene features. Unlike existing methods that use SLAM as initialization, we propose to tightly integrate SLAM and human motion priors in an optimization that is inspired by bundle adjustment. Specifically, we optimize human and camera motions to match both the observed human pose and scene features. This design combines the strengths of SLAM and motion priors, which leads to significant improvements in human and camera motion estimation. We additionally introduce a motion prior that is suitable for batch optimization, making our approach significantly more efficient than existing approaches. Finally, we propose a novel synthetic dataset that enables evaluating camera motion in addition to human motion from dynamic videos. Experiments on the synthetic and real-world RICH datasets demonstrate that our approach substantially outperforms prior art in recovering both human and camera motions.

==> sections/06_supmat.tex <==
\section{Experiments on EgoBody dataset}

EgoBody is a large-scale dataset capturing ground-truth 3D human motions during social interactions in 3D scenes. EgoBody is captured with a head-mounted camera on an interactor, who sees and interacts with a second interactee. The camera moves as the interactor moves, and the ground truth 3D poses of the interactee are recorded in the world coordinate frame. 

We follow~\cite{ye2023slahmr} and use the validation split of the dataset for evaluation. We use DROID-SLAM with the ground-truth camera intrinsics provided by the dataset. 


Table~\ref{tab:egobody_sota} compares \acronym with the state-of-the-art method GLAMR~\cite{yuan2022glamr}. We also compare with the concurrent work SLAHMR~\cite{ye2023slahmr}. As the results indicate, \acronym significantly outperforms GLAMR while achieving performance on par with SLAHMR in terms of accuracy. However, \acronym offers a significant computational advantage over SLAHMR, being up to 50 times faster for a sequence with 1000 frames. Note that the runtime of SLAHMR grows linearly with the sequence length, whereas our runtime increases sub-linearly. This improvement in efficiency demonstrates the potential of \acronym as a practical and effective solution for human and camera motion estimation from videos. 


\section{Global optimization implementation details}
We empirically chose the weights of all error terms involved in the optimization, as summarized in Table~\ref{tab:opt_stages_detailed}. 


\section{HCM dataset generation}
\input{tables/egobody_sota}

To create our HCM (Human and Camera Motion) dataset  we used the characters from the RenderPeople~\cite{renderpeople} dataset with 3D scenes from the Unreal Engine Marketplace~\cite{unreal}. We manually labeled the navigable areas in each 3D scene \ie, sufficiently large, unobstructed flat areas within the scene. To generate a sequence, we randomly selected a 3D scene and a navigable area within it. We also randomly chose the number of people to be animated in the scene, ranging from 1 to 8 individuals. For each person, we selected a motion sequence from the validation set of the AMASS~\cite{AMASS:ICCV:2019} dataset. To ensure that each person's motion sequence was optimized for the scene, we iteratively added one person at a time and optimized their global translation to ensure that they remained within the bounds of the navigable area and did not intersect with existing people in the scene. We also check the terrain height of the navigable area and adjusted each character's root translation accordingly to ensure they were at the correct height relative to the terrain. Finally, we rendered the animated 3D scene into a video sequence using a moving camera. To generate camera trajectories, we designed heuristics
to replicate typical camera movements observed in everyday videos and professional movies. More specifically, we used dolly zoom, random arc motion towards a person, camera motions from the MannequinChallenge dataset~\cite{li2019mannequin}, cameras tracking a specific person, etc. This approach allowed us to generate a diverse set of sequences with varying numbers of people and diverse body and camera motions. In total, we generated 25 video sequences for evaluation. Some examples can be seen in the supplementary video. We believe our HCM dataset will be extremely useful for evaluating human and camera motion estimation methods and furthering research in this direction. 

% \section{Motion prior model}

% NeMF motion prior model explanation here

\input{tables/opt_stages_detailed}


% \section{RICH ablation experiments}
% Table~\ref{tab:rich_ablation} provides the results of the ablation study on the RICH dataset.  We do not provide results for the camera motion estimation since RICH does not provide ground-truth camera poses for the moving camera. The results are mostly consistent with the results on HCM dataset (see Tab.~2 of the main paper). 

==> tables/hcm_ablation.tex <==
% \begin{table}
%     \centering
%     \resizebox{0.47\textwidth}{!}{

%         \begin{tabular}{l|r|r|r|r|r}
%         \toprule
%         \textbf{Methods} & W-MPJPE $\downarrow$ & WA-MPJPE $\downarrow$ & W-RJE $\downarrow$ & PA-MPJPE $\downarrow$ & ACCEL ERR $\downarrow$ \\
%         \midrule 
%         HybrIK-init & 1137.3 & 780.3 & 1100.9 & 67.6 & 51.3 \\
%         GLAMR & 1977.6 & 653.8 & 1958.0 & 86.0 & 33.4 \\
%         stg1 cam & 1110.9 & 650.5 & 1077.3 & 68.4 & 17.2 \\ 
%         stg2 cam zg zl & 982.2 & 484.1 & 946.3 & 68.4 & 18.8 \\
%         stg3 cam zg zl & 970.5 & 483.1 & 937.3 & 66.8 & 17.4 \\
%         stg3 cam zg zl pcl & 863.1 & 474.2 & 838.5 & 64.7 & 16.5 \\ 
%         \bottomrule
%         \end{tabular}
%     }
%    \caption{Ablation experiments on HCM dataset}
%    \label{tab:hcm_ablation}
% \end{table}




\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|r|r|r|r|r|r|r|r}
        \toprule
        & \multicolumn{5}{c|}{\textbf{Human Motion Estimation}} & \multicolumn{3}{c}{\textbf{Camera Motion Estimation}} \\
        \textbf{Methods} & \textbf{\worldErr} $\downarrow$ & \textbf{\worldAlignedErr} $\downarrow$ & \textbf{\worldRootErr} $\downarrow$ & \textbf{\paErr} $\downarrow$ & \textbf{\accel} $\downarrow$ & \textbf{\ate} $\downarrow$ & \textbf{\ateWoS} $\downarrow$ & \textbf{\camAccel} $\downarrow$ \\
        \midrule 
        Initialization & 1116.3 & 650.0 & 1083.1 & 67.6 & 54.3 & 155.8 & 1670.7 & 17.1 \\
        \midrule
        Stage-1 (cam. traj. transform) & 1116.3 & 650.0 & 1083.1 & 67.6 & 54.3 & 155.8 & 643.0 & 17.1 \\
        Stage-2 (+ global human orientation) & 937.0 & 488.2 & 901.9 & 67.6 & 54.6 & 155.8 & 504.9 & 18.1 \\
        Stage-3 (+ local body pose) & 904.5 & 478.2 & 877.9 & 66.6 & 17.6 & 155.8 & 501.3 & 17.3 \\
        Stage-4 (+ full cam. traj.) w/o $E_\textrm{PCL}$ & 870.1 & 487.4 & 844.1 & 67.6 & 53.2 & 166.4 & 505.0 & \textbf{15.4} \\
        \midrule
        HybrIK~\cite{li2020hybrik} + SLAM~\cite{teed2021droid} & 1137.3 & 780.3 & 1100.9 & 67.6 & 51.3 & 155.8 & 1670.7 & 17.1 \\
        GLAMR & 1977.6 & 653.8 & 1958.0 & 86.0 & 33.4 & 1295.2 & 1714.6 & 282.9 \\
        \acronym (Ours) & \textbf{861.2} & \textbf{478.3} & \textbf{839.5} & \textbf{65.3} & \textbf{16.7} & \textbf{137.5} & \textbf{459.7} & 16.2 \\ 
        \bottomrule
        \end{tabular}
    }
   \vspace{-2mm}
   \caption{State-of-the-art comparison and ablation studies on the HCM dataset.}
   \vspace{-4mm}
   \label{tab:hcm_ablation}
\end{table*}


% HybrIK~\cite{li2020hybrik} + SLAM~\cite{teed2021droid} & 1137.3 & 780.3 & 1100.9 & 67.6 & 51.3 & 190.7 & 1658.9 & 17.7 \\
% Initialization (Sec.~\ref{sec:init}) & 1110.9 & 650.5 & 1077.3 & 68.4 & 17.2 & 190.7 & 1658.9 & 17.7 \\
% Non-stagewise opt. & \\
% % stg1 cam & 1110.9 & 650.5 & 1077.3 & 68.4 & 17.2 & 190.7 & 677.7 & 18.5\\ 
% % stg2 cam zg zl & 982.2 & 484.1 & 946.3 & 68.4 & 18.8 & 190.7 & 592.1 & 19.4 \\
% % stg3 cam zg zl & 970.5 & 483.1 & 937.3 & 66.8 & 17.4 & 190.7 & 592.1 & 19.5 \\
% % stg3 cam zg zl pcl & 863.1 & 474.2 & 838.5 & 64.7 & 16.5 & 164.3 & 507.0 & 16.7 \\ 
% Stagewise opt. \\
% \quad Stage 1 & 1110.9 & 650.5 & 1077.3 & 68.4 & 17.2 & 190.7 & 677.7 & 18.5\\ 
% \quad Stage 2 & 982.2 & 484.1 & 946.3 & 68.4 & 18.8 & 190.7 & 592.1 & 19.4 \\
% \quad Stage 3 & 970.5 & 483.1 & 937.3 & 66.8 & 17.4 & 190.7 & 592.1 & 19.5 \\
% % \quad Stage 4  & 863.1 & 474.2 & 838.5 & 64.7 & 16.5 & 164.3 & 507.0 & 16.7 \\
% \quad Stage 4 w/o $E_\textrm{PCL}$  & & & & & & & & \\  
% \midrule
% GLAMR~\cite{yuan2022glamr} & 1977.6 & 653.8 & 1958.0 & 86.0 & 33.4 & 1295.2 & 1714.6 & 282.9\\
% PACE (Ours) & \textbf{863.1} & \textbf{474.2} & \textbf{838.5} & \textbf{64.7} & \textbf{16.5} & \textbf{164.3} & \textbf{507.0} & \textbf{16.7}\\

==> tables/hcm_cam.tex <==

% \begin{table}
%     \centering
%     \resizebox{0.47\textwidth}{!}{

%         \begin{tabular}{l|r|r|r}
%         \toprule
%         \textbf{Methods} & ATE & ATE wo scale & CAM ACCEL \\
%         \midrule 
        
%         HybrIK-init & 190.7 & 1658.9 & 17.7 \\
%         GLAMR & 1295.2 & 1714.6 & 282.9 \\
%         stg1 cam & 190.7 & 677.7 & 18.5 \\
%         stg2 cam zg & 190.7 & 592.1 & 19.4 \\
%         stg3 cam zg zl & 190.7 & 592.1 & 19.5 \\
%         stg3 cam zg zl pcl & 164.3 & 507.0 & 16.7 \\ 
%         \bottomrule
%         \end{tabular} 
%     }

%    \caption{Ablation experiments on HCM dataset}
%     \label{tab:hcm_cam}
% \end{table}

==> tables/hcm_sota.tex <==
% \begin{table}
%     \centering
%     \resizebox{0.47\textwidth}{!}{

%         \begin{tabular}{l|r|r|r|r|r}
%         \toprule
%         \textbf{Methods} & \worldErr \downarrow & \worldAlignedErr \downarrow & \worldRootErr \downarrow & \paErr \downarrow & \accel \downarrow \\
%         \midrule 
%         Initialization & 1137.3 & 780.3 & 1100.9 & 67.6 & 51.3 \\
%         GLAMR & 1977.6 & 653.8 & 1958.0 & 86.0 & 33.4 \\
%         \acronym & 863.1 & 474.2 & 838.5 & 64.7 & 16.5 \\ 
%         \bottomrule
%         \end{tabular}
%     }
%    \caption{State of the art results on HCM dataset}
%    \label{tab:hcm_sota}
% \end{table}

==> tables/rich_ablation.tex <==
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|r|r|r|r|r}
        \toprule
        & \multicolumn{5}{c}{\textbf{Human Motion Estimation}} \\
        \textbf{Methods} & \textbf{\worldErr} $\downarrow$ & \textbf{\worldAlignedErr}$\downarrow$ & \textbf{\worldRootErr} $\downarrow$ & \textbf{\paErr} $\downarrow$ & \textbf{\accel} $\downarrow$ \\
        \midrule 
        Initialization & 579.7 & 343.7 & 571.1 & \textbf{46.7} & 24.3 \\
        \midrule
        Stage-1 & 579.7 & 343.7 & 571.1 & 46.7 & 24.3 \\
        Stage-2 & 427.0 & 210.4 & 413.0 & 46.7 & 23.8 \\
        Stage-3 & 394.7 & 195.7 & 386.1 & 48.5 & 9.6 \\
        % Stage-4 wo $E_\textrm{PCL}$ & \textbf{383.1} & 182.3 & \textbf{369.3} & \textbf{46.7} & 23.0 \\
        % \midrule
        % HybrIK~\cite{li2020hybrik}+SLAM~\cite{teed2021droid} & 1073.1 & 404.4 & 1066.2 & \textbf{46.7} & 20.2 \\
        % GLAMR & 653.7 & 365.1 & 646.6 & 79.9 & 107.7 \\
        % \bf \acronym (Ours) - stage 4 & 387.6 & \textbf{176.3} & 380.1 & 47.5 & \textbf{8.9} \\ 
        \bf \acronym (Ours) - Stage-4 & \textbf{387.6} & \textbf{176.3} & \textbf{380.1} & 47.5 & \textbf{8.9} \\ 
        \bottomrule
        \end{tabular}
    }
    % \vspace{-3mm}
   \caption{Ablation study on the RICH dataset.}
   % \vspace{-4mm}
   \label{tab:rich_ablation}
\end{table}

% \hybrik + SLAM & 1073.1 & 404.4 & 1066.2 & \textbf{46.7} & 20.2 \\
% GLAMR & 653.7 & 365.1 & 646.6 & 79.9 & 107.7 \\
% Initialization & 596.8 & 344.4 & 588.9 & 50.5 & 10.1 \\
% \midrule
% Stage-1 & 596.8 & 344.4 & 588.9 & 50.5 & 10.1 \\
% Stage-2 & 440.6 & 217.5 & 431.1 & 50.5 & 10.4 \\
% Stage-3 & 405.4 & 208.1 & 396.7 & 49.0 & 9.8 \\
% Stage-4 w/o $E_\textrm{PCL}$ &  &  &  &  &  \\ 
% \midrule
% \acronym & \textbf{380.0} & \textbf{197.2} & \textbf{370.8} & 49.3 & \textbf{8.8} \\ 

==> tables/rich_egobody_sota.tex <==
\begin{table*}
    \centering
    \resizebox{0.94\textwidth}{!}{

        \begin{tabular}{l|r|r|r|r|r|r|r|r|r|r}
        \toprule
        & \multicolumn{5}{c|}{Rich Dataset} & \multicolumn{5}{c}{EgoBody Dataset} \\
        \textbf{Methods} & \worldErr \downarrow & \worldAlignedErr\downarrow & \worldRootErr \downarrow & \paErr \downarrow & \accel \downarrow & 
        \worldErr $\downarrow$ & \worldAlignedErr$\downarrow$ & \paErr $\downarrow$ & \accel $\downarrow$ & Runtime (per 1000 imgs)\\
        \midrule 
        % HybrIK + SLAM & - & - & - & - & - \\
        HybrIK + SLAM & 1073.1 & 404.4 & 1066.2 & 46.7 & 20.2 \\
        GLAMR & 653.7 & 365.1 & 646.6 & 79.9 & 107.7 & 416.1 & 239.0 & 114.3 & 173.5 & 7min \\
        SLAHMR & 571.6 & 323.7 & 400.5 & 52.5 & 9.4 & \textbf{141.1} & 101.2 & 79.13 & 25.78 & 400min \\
        \acronym & \textbf{380.0} & \textbf{197.2} & \textbf{370.8} & \textbf{49.3} & \textbf{8.8} &  147.9 & \textbf{101.0} & \textbf{66.5} & \textbf{6.7} & 8min \\ 
        \bottomrule
        \end{tabular}
    }
   \caption{State of the art results on RICH dataset}
   \vspace{-6mm}
   \label{tab:rich_sota}
\end{table*}



% \begin{table}[h]
%     \centering
%     \resizebox{\linewidth}{!}{

%         \begin{tabular}{l|r|r|r|r|r}
%         \toprule
%         \textbf{Methods} & \worldErr $\downarrow$ & \worldAlignedErr$\downarrow$ & \paErr $\downarrow$ & \accel $\downarrow$ & Runtime (per 1000 imgs)\\
%         \midrule 
%         GLAMR~\cite{yuan2022glamr} & 416.1 & 239.0 & 114.3 & 173.5 & 7min \\
%         SLAHMR~\cite{ye2023slahmr} & \textbf{141.1} & 101.2 & 79.13 & 25.78 & 400min \\
%         \acronym (Ours) & 147.9 & \textbf{101.0} & \textbf{66.5} & \textbf{6.7} & 8min \\
%         \bottomrule
%         \end{tabular}
%     }
%    \caption{State-of-the-art results on the EgoBody dataset.}
%    \label{tab:egobody_sota}
% \end{table}

==> tables/rich_sota.tex <==
\begin{table}
    \centering
    \resizebox{0.47\textwidth}{!}{

        \begin{tabular}{l|r|r|r|r|r}
        \toprule
        \textbf{Methods} & \worldErr \downarrow & \worldAlignedErr\downarrow & \worldRootErr \downarrow & \paErr \downarrow & \accel \downarrow \\
        \midrule 
        HybrIK + SLAM & - & - & - & - & - \\
        Initialization & 1073.1 & 404.4 & 1066.2 & 46.7 & 20.2 \\
        GLAMR & 653.7 & 365.1 & 646.6 & 79.9 & 107.7 \\
        \acronym & 380.0 & 197.2 & 370.8 & 49.3 & 8.8 \\ 
        \bottomrule
        \end{tabular}
    }
   \caption{State of the art results on RICH dataset}
   \label{tab:rich_sota}
\end{table}
